Holography as a resource for non-local quantum computation

If two parties share sufficient entanglement, they are able to implement any channel on a shared bipartite state via non-local quantum computation -- a protocol consisting of local operations and a single simultaneous round of quantum communication. Such a protocol can occur in the AdS/CFT correspondence, with the two parties represented by regions of the CFT, and the holographic state serving as a resource to provide the necessary entanglement. This boundary non-local computation is dual to the local implementation of a channel in the bulk AdS theory. Previous work on this phenomenon was obstructed by the divergent entanglement between adjacent CFT regions, and tried to circumvent this issue by assuming that certain regions are irrelevant. However, the absence of these regions introduces violent phenomena that prevent the CFT from implementing the protocol. Instead, we resolve the issue of divergent entanglement by using a finite-memory quantum simulation of the CFT. We show that any finite-memory quantum system on a circular lattice yields a protocol for non-local quantum computation. In the case of a quantum simulation of a holographic CFT, we carefully show that this protocol implements the channel performed by the local bulk dynamics. Under plausible physical assumptions about quantum computation in the bulk, our results imply that non-local quantum computation can be performed for any polynomially complex unitary with a polynomial amount of entanglement. Finally, we provide a concrete example of a holographic code whose bulk dynamics correspond to a Clifford gate, and use our results to show that this corresponds to a non-local quantum computation protocol for this gate.

==> the_lost_section.tex <==
\subsection{How AdS/CFT outperforms existing protocols}

Though the above arguments show that AdS/CFT can perform NLQC more efficiently than existing protocols, the underlying mechanism by which AdS/CFT attains this advantage remains mysterious.
We now argue that the underlying reason for this advantage is that AdS/CFT acts as a ``covariant code'' with a $\mathrm U(1)$ symmetry while previous protocols implicitly use codes with an $\mathrm{SU}(2^n)$ symmetry, which is much more costly.
In particular, a $\mathrm U(1)$ symmetry allows for the resource cost to scale polynomially with the size of the circuit to be implemented.

Loosely speaking, a $G$-covariant code is a code that has a transversal representation of the group $G$.
More formally, a $G$-covariant code  $V:\mathcal{H}_L\rightarrow\mathcal{H}_P=\otimes_{i=1}^m\mathcal{H}_{P_i}$ is an error correcting code with unitary representations
\begin{align*}
    U_L:g&\rightarrow \text{Unitary}(\mathcal{H}_L)\\
    U_P:g&\rightarrow \text{Unitary}(\mathcal{H}_P).
\end{align*}
such that for all $g\in G$ we have $U_P(g)V=VU_L(g)$ and each $U_P(g)$ is a tensor product of local operators on each physical site, i.e.\ $U_P(g)= \otimes_{i=1}^mU_{P_i}(g)$.
It is well-known that if $V$ can perfectly correct non-trivial erasure errors, than the group $G$ must be finite \cite{Eastin_2009}. 
However, if $V$ acts only approximately as an error correcting code -- the recovery introduces noise -- then $G$ can be made continuous \cite{Faist}. 
For the error to go to zero, the number of physical sites or their local dimension must be large.
In particular, suppose $\mathcal{H}_L$ has dimension $d_L$ and that $\mathcal{H}_{P_i}$ has dimension $d$.
It is shown in \cite{Faist} that if $G=\mathrm{SU}(d_L)$, $U_L$ is the defining representation (i.e. $U_L(G)$ is a universal gate set), and $m$ is fixed, then $d\sim \exp(d_L)$ in order for the code to remain accurate. 
On the other hand, it is simple to construct accurate $\mathrm{U}(1)$ covariant codes where $U_L$ acts non-trivially on all logical states and in which $d\sim \mathrm{poly}(d_L)$.

In the most efficient known NLQC protocol which works for all unitaries \cite{beigi-koenig}, a crucial step involves Alice ``port-teleporting'' $n$ qubits to Bob \cite{port-teleportation}. 
To do this, Alice and Bob must share as a resource $N$ sets, called ``ports'', of $n$ Bell pairs. Alice then performs some POVM on the $n$ qubits and her half of the ports, and as a result measures some number $x\in\{1,...,N\}$. 
The state of the $n$ qubits is then instantly transferred to Bob's half of the $x$th port, much like in normal teleportation, but without Pauli corrections. Superluminal signalling is not violated, because Bob does not know the value of $x$. 
The advantage of port-based teleportation is that Bob can perform any unitary on the $n$ qubits \textit{before} receiving the value of $x$ by acting with the same unitary on all ports. 
However, this same advantage -- transversality of $\mathrm{SU}(2^n)$ -- makes port teleportation very costly. 
If $N$ is large and Bob discards a small number of his halves of the ports, it is unlikely that he will throw away the $x$th port.
Therefore he can probably correct a non-trivial erasure, so port-teleportation acts as an approximate $\mathrm{SU}(2^n)$ covariant code.
Thus port teleportation can only be accurate in the regime if the physical dimension $d$ is exponentially large in the dimension of the logical space $d_L$, i.e.\ $N$ is exponential in $n$.
Hence, the reason previous protocols are inefficient is that they distribute resources that act as an $\mathrm{SU}(2^n)$ covariant code. 

On the other hand, for a low energy subspace, we may view AdS/CFT as a $\mathrm U(1)$ covariant code in which $U_L(t)=e^{-iH_{bulk} t}$ and $U_P(t)=e^{-iH_{CFT} t}$\footnote{Here the physical unitaries are of the more general form of being generated by a local Hamiltonian rather than being product. The results of \cite{Faist} address this as well.}. 
For a given $H_{bulk}$, $\{U_L(t)\}_t$ must be a proper subset of all unitaries acting on $L$.
However, it is possible for $U_L$ to act as any unitary achievable by a universal quantum computer with finite program memory and computational time.
In this way, the set $\{U_L(t)\}_t$ includes all low-complexity unitaries -- analogous to a space-filling curve.
We now demonstrate this claim with a concrete example, and then explain how this example can be embedded directly into holography.
%That is, one can embed $\mathrm{U}(1)$ in such a way that it 

As an example of how a $U(1)$ subgroup can act as such a universal quantum computer with limited resources, consider one that is generated by a Feynman-Kitaev clock Hamiltonian (see \cite{Jordan_2017} for example).
This Hamiltonian implements a particular quantum circuit $C$ on a subset of its input qubits, with the rest serving as ancillas.
The number of ancillas is polynomial in the number of $2$-qubit gates in the circuit to be implemented, i.e.\ the ``size'' of that circuit.
If we choose the circuit to read the first $m$ qubits of the input states, and if they are in the computational basis state $k\in \{0,1\}^{m}$ apply a circuit $C_k$ on the remaining $n$ qubits, this models a computer with an $m$-bit program memory.
Furthermore, clearly the size of each $C_k$ is also limited by the number of ancillas that the clock Hamiltonian may act on, thus modelling a computer that can run for only a finite time.
Thus any circuit can be implemented, with the number of resources scaling polynomially with the circuit size, just as the arguments in the previous subsections would suggest. 

A distinction here is that, whereas the $SU$ approach is directly compatible with transversality of any unitary, the unitaries for which $U(1)$ covariance works is dependent on the initial state.
This can be seen explicitly by the role of the program memory in the example above.
In our holographic construction, the resource state similarly encodes the unitary to be implemented, as the bulk dynamics are determined by the initial CFT state.
To be honest this makes it unclear if U(1) covariance is really that useful of a mechanism -- i.e., is that really what holography is doing?
